Market Interventions in a Large-Scale Virtual Economy

Massively multiplayer online role-playing games often contain sophisticated in-game economies. Many important real-world economic phenomena, such as inflation, economic growth, and business cycles, are also present in these virtual economies. One major difference between real-world and virtual economies is the ease and frequency by which a policymaker, in this case, a game developer, can introduce economic shocks. These economic shocks, typically implemented with game updates or signaled through community channels, provide fertile ground to study the effects of economic interventions on markets. In this work, we study the effect of in-game economic market interventions, namely, a transaction tax and an item sink, in Old School RuneScape. Using causal inference methods, we find that the tax did not meaningfully affect the trading volume of items at the tax boundaries and that the item sink contributed to the inflation of luxury good prices, without reducing trade volume. Furthermore, we find evidence that the illicit gold trading market was relatively unaffected by the implemented market interventions. Our findings yield useful insights not only into the effect of market interventions in virtual economies but also for real-world markets.

==> 00_ge_tax_ideas.tex <==
Potential ideas:
- effect of tax on item liquidity
- effect of tax on market structure (PROBABLY NOT)
- Document the disinflation of luxury goods (pre-tax imposition)
- effect of sink on expensive goods by comparing price change for similar (but not sinked) goods [is this a causal inference ting?] ***********  Needs careful definition of similar goods (no it doesnt)


Structure:
Section 1. Intro
Section 2. Related Work
Section 3. Dataset/Game explanation, EDA
explaining economy structure, Explain the key interesting trends (disinflation of end-game goods) (player counts as a possible indicator of botting?)
Section 4. Document the effects of the policy change
(causal analysis and liquidity) (also document effect on gold selling) (effect of financial tax on volume + gold price + membership bond price)
Section 5. Discussion
implications for real-world markets, other online markets.  Discussion of financial tax proprosals in the EU
Section 6. Conclusion

To-do:
Intro/RW/Data & Markets - Peter
Iron out causal model for items around the tax cutoffs

Action Items (Peter):
- Start writing abstract/intro/RW/dataset

Action Items (Senan):
- Look into options for similar (not sinked) goods, which are not substitutes or complements (use network analysis of to inform which are similar goods)
- Iron out causal effects



==> 00_notes.tex <==
Analyzing Uber’s Ride-sharing Economy looks like a good paper to model after

No Silk Road for Online Gamers!: Using Social Network Analysis to Unveil Black Markets in Online Games - black market stuff

Achievement and Friends: Key Factors of Player Retention Vary Across Player Levels in Online Multiplayer Games

Rise and Fall of Online Game Groups: Common Findings on Two Different Games - study of rise and fall of mmos

Unveiling group characteristics in online social games: a socio-economic analysis

I Would Not Plant Apple Trees If the World Will Be Wiped: Analyzing Hundreds of Millions of Behavioral Records of Players During an MMORPG Beta Test - big scale MMORPG, incentives

Game over? Negotiating modern capitalism in virtual game worlds - virtual marketplace in WoW, etc., colonization, RWT

VIRTUAL ECONOMICS: APPLYING ECONOMICS TO THE STUDY OF GAME WORLDS - mmorpgs to study economics

On Virtual Economies - old old virtual economies paper

REAL ECONOMICS IN VIRTUAL WORLDS: A MASSIVELY MULTIPLAYER ONLINE GAME CASE STUDY, RUNESCAPE - masters thesis on it

Examining the effects of network externalities, density, and closure on in-game currency price in online games - currency prices in online games

Epic, Steam, and the role of skin-betting in game (platform) economies - speculation 

You Are a Game Bot!: Uncovering Game Bots in MMORPGs via Self-similarity in the Wild - bot detection

Spending Real Money: Purchasing Patterns of Virtual Goods in an Online Social Game - purchasing patterns real world to virtual

A Brief History of Virtual Economy - history of 

As real as real? Macroeconomic behavior in a large-scale virtual world

Analysis of the Relationship between Virtual Goods Trading and Performance of Virtual Worlds 

The Gift That Keeps on Giving: Generosity is Contagious in Multiplayer Online Games

Niko Lahti
Inflation Control in Virtual Economies

Synthetic Worlds
The Business and Culture of Online Games
Edward Castronova

Advances in Measuring Inflation Within Virtual Economies Using Deep Reinforcement Learning

Study on the Inflation in the Economic System in Online Games

On the connection between real-world circumstances and online player behaviour: The case of EVE Online

https://www.pcgamer.com/amazon-says-new-worlds-economy-is-just-fine-thanks/
https://www.inputmag.com/gaming/amazons-new-world-is-suffering-from-a-bizarre-currency-crisis

% https://en.wikipedia.org/wiki/File:Illustration_of_Difference_in_Differences
% https://en.wikipedia.org/wiki/Difference_in_differences

WWW:
The scope of the conference is the Web and how it has crucially enabled new research and applications. While the Web feeds on and is part of a broader interdisciplinary ecosystem, including technologies such as machine learning, natural language processing, computer vision, and many others, it remains a distinct scholarly field, with its own research methods, tools, and challenges.
As such, submissions that merely use one or another Web artifact — e.g., a dataset or a Web Application Programmer


==> 00_reference_notes.tex <==
\cite{castronova2001virtual} makes reference to the virtual currency/RMT trade
